A New Class of Compact Formulations for Vehicle Routing Problems

This paper introduces a novel compact mixed integer linear programming (MILP) formulation and a discretization discovery-based solution approach for the Vehicle Routing Problem with Time Windows (VRPTW). We aim to solve the optimization problem efficiently by constraining the linear programming (LP) solutions to use only flows corresponding to time and capacity-feasible routes that are locally elementary (prohibiting cycles of customers localized in space). We employ a discretization discovery algorithm to refine the LP relaxation iteratively. This iterative process alternates between two steps: (1) increasing time/capacity/elementarity enforcement to increase the LP objective, albeit at the expense of increased complexity (more variables and constraints), and (2) decreasing enforcement without decreasing the LP objective to reduce complexity. This iterative approach ensures we produce an LP relaxation that closely approximates the optimal MILP objective with minimal complexity, facilitating an efficient solution via an off-the-shelf MILP solver. The effectiveness of our method is demonstrated through empirical evaluations on classical VRPTW instances. We showcase the efficiency of solving the final MILP and multiple iterations of LP relaxations, highlighting the decreased integrality gap of the final LP relaxation. We believe that our approach holds promise for addressing a wide range of routing problems within and beyond the VRPTW domain.

==> bene_results/bene_graph_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_c100.tex <==
\begin{table}
\centering
\caption{Improvment via Graph Choice:   Num Customers = 50 Problem Set = c100}
\label{tabGraph:50Problem Set=c100}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time  \\
\midrule
c101 & None; BASELINE MILP & 362 & 363 & 363 & 0 & 0 \\
c101 & None & 362 & 363 & 363 & 0 & 0 \\
c101 & time & 363 & 363 & 363 & 0 & 0 \\
c101 & demand & 363 & 363 & 363 & 0 & 0 \\
c101 & both & 363 & 363 & 363 & 0 & 1 \\
c102 & None; BASELINE MILP & 335 & 362 & 362 & 1 & 0 \\
c102 & None & 352 & 362 & 362 & 1 & 0 \\
c102 & time & 362 & 362 & 362 & 0 & 1 \\
c102 & demand & 361 & 362 & 362 & 1 & 14 \\
c102 & both & 362 & 362 & 362 & 0 & 3 \\
c103 & None; BASELINE MILP & 285 & 362 & 362 & 30 & 0 \\
c103 & None & 329 & 362 & 362 & 11 & 0 \\
c103 & time & 357 & 362 & 362 & 1 & 7 \\
c103 & demand & 355 & 362 & 362 & 23 & 33 \\
c103 & both & 362 & 362 & 362 & 1 & 37 \\
c104 & None; BASELINE MILP & 282 & 316 & 359 & 1000 & 0 \\
c104 & None & 299 & 319 & 359 & 1000 & 0 \\
c104 & time & 351 & 359 & 359 & 25 & 39 \\
c104 & demand & 347 & 359 & 359 & 339 & 53 \\
c104 & both & 356 & 359 & 359 & 12 & 74 \\
c105 & None; BASELINE MILP & 361 & 363 & 363 & 0 & 0 \\
c105 & None & 362 & 363 & 363 & 0 & 0 \\
c105 & time & 362 & 363 & 363 & 0 & 0 \\
c105 & demand & 362 & 363 & 363 & 0 & 1 \\
c105 & both & 363 & 363 & 363 & 0 & 1 \\
c106 & None; BASELINE MILP & 361 & 363 & 363 & 0 & 0 \\
c106 & None & 362 & 363 & 363 & 0 & 0 \\
c106 & time & 363 & 363 & 363 & 0 & 0 \\
c106 & demand & 363 & 363 & 363 & 0 & 1 \\
c106 & both & 363 & 363 & 363 & 0 & 1 \\
c107 & None; BASELINE MILP & 361 & 363 & 363 & 0 & 0 \\
c107 & None & 362 & 363 & 363 & 0 & 0 \\
c107 & time & 362 & 363 & 363 & 0 & 0 \\
c107 & demand & 363 & 363 & 363 & 0 & 1 \\
c107 & both & 363 & 363 & 363 & 0 & 1 \\
c108 & None; BASELINE MILP & 262 & 363 & 363 & 1 & 0 \\
c108 & None & 354 & 363 & 363 & 1 & 0 \\
c108 & time & 362 & 363 & 363 & 0 & 2 \\
c108 & demand & 363 & 363 & 363 & 2 & 25 \\
c108 & both & 363 & 363 & 363 & 0 & 7 \\
c109 & None; BASELINE MILP & 258 & 363 & 363 & 22 & 0 \\
c109 & None & 335 & 363 & 363 & 8 & 0 \\
c109 & time & 359 & 363 & 363 & 2 & 13 \\
c109 & demand & 360 & 363 & 363 & 7 & 80 \\
c109 & both & 363 & 363 & 363 & 2 & 44 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_graph_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_c200.tex <==
\begin{table}
\centering
\caption{Improvment via Graph Choice:   Num Customers = 50 Problem Set = c200}
\label{tabGraph:50Problem Set=c200}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time  \\
\midrule
c201 & None; BASELINE MILP & 362 & 362 & 362 & 0 & 0 \\
c201 & None & 362 & 362 & 362 & 0 & 0 \\
c201 & time & 362 & 362 & 362 & 0 & 0 \\
c201 & demand & 362 & 362 & 362 & 0 & 1 \\
c201 & both & 362 & 362 & 362 & 0 & 1 \\
c202 & None; BASELINE MILP & 320 & 362 & 362 & 2 & 0 \\
c202 & None & 347 & 362 & 362 & 2 & 0 \\
c202 & time & 362 & 362 & 362 & 0 & 4 \\
c202 & demand & 347 & 362 & 362 & 2 & 6 \\
c202 & both & 362 & 362 & 362 & 0 & 11 \\
c203 & None; BASELINE MILP & 300 & 342 & 361 & 12 & 0 \\
c203 & None & 341 & 361 & 361 & 6 & 0 \\
c203 & time & 361 & 361 & 361 & 0 & 23 \\
c203 & demand & 341 & 361 & 361 & 4 & 9 \\
c203 & both & 361 & 361 & 361 & 0 & 33 \\
c204 & None; BASELINE MILP & 290 & 346 & 352 & 1000 & 0 \\
c204 & None & 326 & 349 & 352 & 1000 & 0 \\
c204 & time & 352 & 352 & 352 & 1 & 47 \\
c204 & demand & 326 & 349 & 352 & 1000 & 11 \\
c204 & both & 352 & 352 & 352 & 2 & 72 \\
c205 & None; BASELINE MILP & 314 & 361 & 361 & 0 & 0 \\
c205 & None & 361 & 361 & 361 & 0 & 0 \\
c205 & time & 361 & 361 & 361 & 0 & 1 \\
c205 & demand & 361 & 361 & 361 & 0 & 2 \\
c205 & both & 361 & 361 & 361 & 0 & 3 \\
c206 & None; BASELINE MILP & 312 & 361 & 361 & 1 & 0 \\
c206 & None & 361 & 361 & 361 & 0 & 0 \\
c206 & time & 361 & 361 & 361 & 0 & 1 \\
c206 & demand & 361 & 361 & 361 & 0 & 3 \\
c206 & both & 361 & 361 & 361 & 0 & 3 \\
c207 & None; BASELINE MILP & 312 & 361 & 361 & 2 & 0 \\
c207 & None & 345 & 361 & 361 & 3 & 0 \\
c207 & time & 358 & 361 & 361 & 2 & 41 \\
c207 & demand & 345 & 361 & 361 & 2 & 9 \\
c207 & both & 358 & 361 & 361 & 1 & 56 \\
c208 & None; BASELINE MILP & 310 & 352 & 352 & 1 & 0 \\
c208 & None & 345 & 352 & 352 & 0 & 0 \\
c208 & time & 349 & 352 & 352 & 0 & 2 \\
c208 & demand & 345 & 352 & 352 & 1 & 4 \\
c208 & both & 349 & 352 & 352 & 1 & 9 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_graph_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_r100.tex <==
\begin{table}
\centering
\caption{Improvment via Graph Choice:   Num Customers = 50 Problem Set = r100}
\label{tabGraph:50Problem Set=r100}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time  \\
\midrule
r101 & None; BASELINE MILP & 1032 & 1047 & 1047 & 0 & 0 \\
r101 & None & 1041 & 1047 & 1047 & 0 & 0 \\
r101 & time & 1047 & 1047 & 1047 & 0 & 0 \\
r101 & demand & 1041 & 1047 & 1047 & 0 & 0 \\
r101 & both & 1047 & 1047 & 1047 & 0 & 0 \\
r102 & None; BASELINE MILP & 652 & 911 & 911 & 51 & 0 \\
r102 & None & 737 & 911 & 911 & 87 & 0 \\
r102 & time & 911 & 911 & 911 & 0 & 0 \\
r102 & demand & 744 & 911 & 911 & 391 & 25 \\
r102 & both & 911 & 911 & 911 & 0 & 1 \\
r103 & None; BASELINE MILP & 536 & 726 & 776 & 1000 & 0 \\
r103 & None & 601 & 741 & 776 & 1000 & 0 \\
r103 & time & 765 & 776 & 776 & 2 & 9 \\
r103 & demand & 625 & 703 & 778 & 1000 & 32 \\
r103 & both & 765 & 776 & 776 & 2 & 11 \\
r104 & None; BASELINE MILP & 467 & 545 & 653 & 1000 & 0 \\
r104 & None & 508 & 545 & 653 & 1000 & 0 \\
r104 & time & 615 & 631 & 631 & 65 & 36 \\
r104 & demand & 555 & 565 & 653 & 1000 & 48 \\
r104 & both & 615 & 631 & 631 & 53 & 75 \\
r105 & None; BASELINE MILP & 795 & 914 & 914 & 1 & 0 \\
r105 & None & 864 & 914 & 914 & 1 & 0 \\
r105 & time & 901 & 914 & 914 & 0 & 0 \\
r105 & demand & 864 & 914 & 914 & 1 & 1 \\
r105 & both & 901 & 914 & 914 & 0 & 1 \\
r106 & None; BASELINE MILP & 549 & 795 & 795 & 629 & 0 \\
r106 & None & 637 & 795 & 795 & 365 & 0 \\
r106 & time & 795 & 795 & 795 & 0 & 2 \\
r106 & demand & 660 & 745 & 795 & 1000 & 49 \\
r106 & both & 795 & 795 & 795 & 0 & 4 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_graph_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_r100pt2.tex <==
\begin{table}
\centering
\caption{Improvment via Graph Choice:   Num Customers = 50 Problem Set = r100pt2}
\label{tabGraph:50Problem Set=r100pt2}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time  \\
\midrule
r107 & None; BASELINE MILP & 486 & 634 & 714 & 1000 & 0 \\
r107 & None & 541 & 646 & 714 & 1000 & 0 \\
r107 & time & 703 & 714 & 714 & 4 & 13 \\
r107 & demand & 586 & 630 & 717 & 1000 & 56 \\
r107 & both & 703 & 714 & 714 & 2 & 30 \\
r108 & None; BASELINE MILP & 460 & 533 & 634 & 1000 & 0 \\
r108 & None & 500 & 535 & 633 & 1000 & 0 \\
r108 & time & 587 & 608 & 620 & 1000 & 52 \\
r108 & demand & 551 & 562 & 624 & 1000 & 62 \\
r108 & both & 587 & 606 & 620 & 1000 & 106 \\
r109 & None; BASELINE MILP & 550 & 771 & 791 & 1000 & 0 \\
r109 & None & 654 & 791 & 791 & 977 & 0 \\
r109 & time & 755 & 791 & 791 & 14 & 11 \\
r109 & demand & 658 & 738 & 794 & 1000 & 41 \\
r109 & both & 755 & 791 & 791 & 14 & 38 \\
r110 & None; BASELINE MILP & 483 & 613 & 699 & 1000 & 0 \\
r110 & None & 552 & 624 & 699 & 1000 & 0 \\
r110 & time & 684 & 699 & 699 & 8 & 29 \\
r110 & demand & 577 & 600 & 721 & 1000 & 68 \\
r110 & both & 683 & 699 & 699 & 13 & 36 \\
r111 & None; BASELINE MILP & 478 & 608 & 711 & 1000 & 0 \\
r111 & None & 539 & 620 & 717 & 1000 & 0 \\
r111 & time & 677 & 710 & 710 & 23 & 24 \\
r111 & demand & 586 & 614 & 731 & 1000 & 52 \\
r111 & both & 677 & 710 & 710 & 22 & 38 \\
r112 & None; BASELINE MILP & 455 & 520 & 655 & 1000 & 0 \\
r112 & None & 491 & 511 & 647 & 1000 & 0 \\
r112 & time & 597 & 617 & 638 & 1000 & 69 \\
r112 & demand & 543 & 545 & 652 & 1000 & 53 \\
r112 & both & 597 & 618 & 633 & 1000 & 166 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_graph_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_r200.tex <==
\begin{table}
\centering
\caption{Improvment via Graph Choice:   Num Customers = 50 Problem Set = r200}
\label{tabGraph:50Problem Set=r200}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time  \\
\midrule
r201 & None; BASELINE MILP & 703 & 794 & 794 & 0 & 0 \\
r201 & None & 789 & 794 & 794 & 0 & 0 \\
r201 & time & 792 & 794 & 794 & 0 & 1 \\
r201 & demand & 789 & 794 & 794 & 0 & 3 \\
r201 & both & 792 & 794 & 794 & 0 & 3 \\
r202 & None; BASELINE MILP & 507 & 685 & 701 & 1000 & 0 \\
r202 & None & 597 & 682 & 701 & 1000 & 0 \\
r202 & time & 683 & 701 & 701 & 7 & 27 \\
r202 & demand & 597 & 692 & 701 & 1000 & 21 \\
r202 & both & 683 & 701 & 701 & 5 & 77 \\
r203 & None; BASELINE MILP & 451 & 539 & 608 & 1000 & 0 \\
r203 & None & 502 & 549 & 608 & 1000 & 0 \\
r203 & time & 572 & 608 & 608 & 47 & 39 \\
r203 & demand & 502 & 552 & 608 & 1000 & 35 \\
r203 & both & 573 & 608 & 608 & 52 & 179 \\
r204 & None; BASELINE MILP & 423 & 478 & 511 & 1000 & 0 \\
r204 & None & 460 & 480 & 515 & 1000 & 0 \\
r204 & time & 467 & 486 & 511 & 1000 & 80 \\
r204 & demand & 460 & 479 & 511 & 1000 & 21 \\
r204 & both & 467 & 488 & 511 & 1000 & 247 \\
r205 & None; BASELINE MILP & 543 & 692 & 692 & 74 & 0 \\
r205 & None & 647 & 692 & 692 & 98 & 0 \\
r205 & time & 664 & 692 & 692 & 8 & 16 \\
r205 & demand & 647 & 692 & 692 & 24 & 11 \\
r205 & both & 664 & 692 & 692 & 5 & 70 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_graph_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_r200pt2.tex <==
\begin{table}
\centering
\caption{Improvment via Graph Choice:   Num Customers = 50 Problem Set = r200pt2}
\label{tabGraph:50Problem Set=r200pt2}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time  \\
\midrule
r206 & None; BASELINE MILP & 458 & 588 & 649 & 1000 & 0 \\
r206 & None & 543 & 592 & 635 & 1000 & 0 \\
r206 & time & 587 & 635 & 635 & 314 & 75 \\
r206 & demand & 543 & 593 & 641 & 1000 & 47 \\
r206 & both & 587 & 635 & 635 & 513 & 220 \\
r207 & None; BASELINE MILP & 423 & 522 & 602 & 1000 & 0 \\
r207 & None & 488 & 529 & 581 & 1000 & 0 \\
r207 & time & 522 & 558 & 579 & 1000 & 132 \\
r207 & demand & 488 & 530 & 579 & 1000 & 42 \\
r207 & both & 522 & 560 & 578 & 1000 & 369 \\
r208 & None; BASELINE MILP & 415 & 472 & 505 & 1000 & 0 \\
r208 & None & 457 & 474 & 501 & 1000 & 0 \\
r208 & time & 457 & 471 & 497 & 1000 & 18 \\
r208 & demand & 457 & 474 & 490 & 1000 & 24 \\
r208 & both & 457 & 471 & 495 & 1000 & 73 \\
r209 & None; BASELINE MILP & 484 & 603 & 603 & 374 & 0 \\
r209 & None & 553 & 603 & 603 & 349 & 0 \\
r209 & time & 571 & 603 & 603 & 49 & 53 \\
r209 & demand & 553 & 603 & 603 & 104 & 20 \\
r209 & both & 571 & 603 & 603 & 94 & 140 \\
r210 & None; BASELINE MILP & 458 & 601 & 650 & 1000 & 0 \\
r210 & None & 548 & 602 & 655 & 1000 & 0 \\
r210 & time & 596 & 639 & 648 & 1000 & 73 \\
r210 & demand & 548 & 606 & 660 & 1000 & 17 \\
r210 & both & 596 & 648 & 648 & 824 & 171 \\
r211 & None; BASELINE MILP & 415 & 482 & 549 & 1000 & 0 \\
r211 & None & 457 & 479 & 568 & 1000 & 0 \\
r211 & time & 492 & 515 & 538 & 1000 & 178 \\
r211 & demand & 457 & 476 & 561 & 1000 & 22 \\
r211 & both & 492 & 511 & 538 & 1000 & 501 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_graph_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_rc100.tex <==
\begin{table}
\centering
\caption{Improvment via Graph Choice:   Num Customers = 50 Problem Set = rc100}
\label{tabGraph:50Problem Set=rc100}
\begin{tabular}{}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time  \\
\midrule
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_graph_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_rc200.tex <==
\begin{table}
\centering
\caption{Improvment via Graph Choice:   Num Customers = 50 Problem Set = rc200}
\label{tabGraph:50Problem Set=rc200}
\begin{tabular}{}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time  \\
\midrule
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_la_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_c100.tex <==
\begin{table}
\centering
\caption{Improvment via LA Choice:   Num Customers = 50 Problem Set = c100}
\label{tabLA:50Problem Set=c100}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time   \\
\midrule
c101 & BASELINE MILP & 362.2 & 363.2 & 363.2 & 0.0 & 0.0 \\
c101 & 0 & 363.2 & 363.2 & 363.2 & 0.0 & 0.8 \\
c101 & 2 & 363.2 & 363.2 & 363.2 & 0.0 & 0.6 \\
c101 & 4 & 363.2 & 363.2 & 363.2 & 0.0 & 0.7 \\
c101 & 6 & 363.2 & 363.2 & 363.2 & 0.0 & 0.7 \\
c102 & BASELINE MILP & 334.8 & 362.2 & 362.2 & 0.5 & 0.0 \\
c102 & 0 & 361.0 & 362.2 & 362.2 & 0.2 & 3.2 \\
c102 & 2 & 362.2 & 362.2 & 362.2 & 0.2 & 1.7 \\
c102 & 4 & 362.2 & 362.2 & 362.2 & 0.1 & 2.3 \\
c102 & 6 & 362.2 & 362.2 & 362.2 & 0.1 & 2.6 \\
c103 & BASELINE MILP & 285.5 & 362.2 & 362.2 & 30.2 & 0.0 \\
c103 & 0 & 361.0 & 362.2 & 362.2 & 2.1 & 26.9 \\
c103 & 2 & 362.2 & 362.2 & 362.2 & 0.9 & 26.9 \\
c103 & 4 & 362.2 & 362.2 & 362.2 & 0.7 & 34.6 \\
c103 & 6 & 362.2 & 362.2 & 362.2 & 0.9 & 37.0 \\
c104 & BASELINE MILP & 281.7 & 316.5 & 358.9 & 1000.0 & 0.0 \\
c104 & 0 & 353.0 & 358.9 & 358.9 & 33.0 & 50.8 \\
c104 & 2 & 356.0 & 358.9 & 358.9 & 10.1 & 67.2 \\
c104 & 4 & 356.0 & 358.9 & 358.9 & 12.9 & 70.5 \\
c104 & 6 & 356.0 & 358.9 & 358.9 & 12.1 & 73.9 \\
c105 & BASELINE MILP & 360.8 & 363.2 & 363.2 & 0.1 & 0.0 \\
c105 & 0 & 363.2 & 363.2 & 363.2 & 0.1 & 1.0 \\
c105 & 2 & 363.2 & 363.2 & 363.2 & 0.0 & 1.0 \\
c105 & 4 & 362.9 & 363.2 & 363.2 & 0.1 & 0.9 \\
c105 & 6 & 363.2 & 363.2 & 363.2 & 0.0 & 1.0 \\
c106 & BASELINE MILP & 360.9 & 363.2 & 363.2 & 0.1 & 0.0 \\
c106 & 0 & 363.2 & 363.2 & 363.2 & 0.1 & 0.6 \\
c106 & 2 & 363.2 & 363.2 & 363.2 & 0.1 & 0.9 \\
c106 & 4 & 363.2 & 363.2 & 363.2 & 0.1 & 0.8 \\
c106 & 6 & 363.2 & 363.2 & 363.2 & 0.1 & 0.9 \\
c107 & BASELINE MILP & 360.8 & 363.2 & 363.2 & 0.1 & 0.0 \\
c107 & 0 & 362.9 & 363.2 & 363.2 & 0.1 & 1.1 \\
c107 & 2 & 363.2 & 363.2 & 363.2 & 0.1 & 1.7 \\
c107 & 4 & 362.9 & 363.2 & 363.2 & 0.1 & 1.0 \\
c107 & 6 & 362.9 & 363.2 & 363.2 & 0.1 & 1.1 \\
c108 & BASELINE MILP & 261.8 & 363.2 & 363.2 & 0.8 & 0.0 \\
c108 & 0 & 362.7 & 363.2 & 363.2 & 0.3 & 20.6 \\
c108 & 2 & 363.2 & 363.2 & 363.2 & 0.2 & 6.3 \\
c108 & 4 & 363.2 & 363.2 & 363.2 & 0.3 & 6.6 \\
c108 & 6 & 363.2 & 363.2 & 363.2 & 0.2 & 7.1 \\
c109 & BASELINE MILP & 257.8 & 363.2 & 363.2 & 21.8 & 0.0 \\
c109 & 0 & 358.0 & 363.2 & 363.2 & 4.0 & 53.9 \\
c109 & 2 & 362.5 & 363.2 & 363.2 & 3.3 & 63.8 \\
c109 & 4 & 362.6 & 363.2 & 363.2 & 1.9 & 42.4 \\
c109 & 6 & 362.6 & 363.2 & 363.2 & 1.8 & 44.3 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_la_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_c200.tex <==
\begin{table}
\centering
\caption{Improvment via LA Choice:   Num Customers = 50 Problem Set = c200}
\label{tabLA:50Problem Set=c200}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time   \\
\midrule
c201 & BASELINE MILP & 361.8 & 361.8 & 361.8 & 0.0 & 0.0 \\
c201 & 0 & 361.8 & 361.8 & 361.8 & 0.0 & 0.9 \\
c201 & 2 & 361.8 & 361.8 & 361.8 & 0.0 & 0.9 \\
c201 & 4 & 361.8 & 361.8 & 361.8 & 0.0 & 0.7 \\
c201 & 6 & 361.8 & 361.8 & 361.8 & 0.0 & 1.0 \\
c202 & BASELINE MILP & 319.5 & 361.8 & 361.8 & 2.1 & 0.0 \\
c202 & 0 & 361.8 & 361.8 & 361.8 & 0.1 & 4.2 \\
c202 & 2 & 361.8 & 361.8 & 361.8 & 0.1 & 4.6 \\
c202 & 4 & 361.8 & 361.8 & 361.8 & 0.1 & 5.4 \\
c202 & 6 & 361.8 & 361.8 & 361.8 & 0.1 & 11.2 \\
c203 & BASELINE MILP & 300.4 & 341.8 & 361.4 & 11.9 & 0.0 \\
c203 & 0 & 361.1 & 361.4 & 361.4 & 0.9 & 28.0 \\
c203 & 2 & 361.4 & 361.4 & 361.4 & 0.2 & 21.7 \\
c203 & 4 & 361.4 & 361.4 & 361.4 & 0.2 & 19.5 \\
c203 & 6 & 361.4 & 361.4 & 361.4 & 0.2 & 32.7 \\
c204 & BASELINE MILP & 290.0 & 345.6 & 351.7 & 1000.0 & 0.0 \\
c204 & 0 & 345.8 & 351.7 & 351.7 & 6.4 & 70.4 \\
c204 & 2 & 351.5 & 351.7 & 351.7 & 0.8 & 56.0 \\
c204 & 4 & 351.5 & 351.7 & 351.7 & 0.8 & 41.4 \\
c204 & 6 & 351.5 & 351.7 & 351.7 & 1.7 & 71.7 \\
c205 & BASELINE MILP & 314.5 & 361.4 & 361.4 & 0.2 & 0.0 \\
c205 & 0 & 342.7 & 361.4 & 361.4 & 0.2 & 5.7 \\
c205 & 2 & 361.4 & 361.4 & 361.4 & 0.1 & 2.2 \\
c205 & 4 & 361.4 & 361.4 & 361.4 & 0.1 & 3.4 \\
c205 & 6 & 361.4 & 361.4 & 361.4 & 0.1 & 2.7 \\
c206 & BASELINE MILP & 312.2 & 361.4 & 361.4 & 0.9 & 0.0 \\
c206 & 0 & 339.4 & 361.4 & 361.4 & 0.4 & 14.1 \\
c206 & 2 & 359.9 & 361.4 & 361.4 & 0.2 & 11.4 \\
c206 & 4 & 359.4 & 361.4 & 361.4 & 0.1 & 4.5 \\
c206 & 6 & 361.4 & 361.4 & 361.4 & 0.1 & 3.2 \\
c207 & BASELINE MILP & 312.0 & 361.2 & 361.2 & 2.0 & 0.0 \\
c207 & 0 & 349.3 & 361.2 & 361.2 & 4.2 & 35.4 \\
c207 & 2 & 357.0 & 361.2 & 361.2 & 2.8 & 40.0 \\
c207 & 4 & 358.3 & 361.2 & 361.2 & 1.9 & 52.5 \\
c207 & 6 & 358.2 & 361.2 & 361.2 & 1.4 & 56.3 \\
c208 & BASELINE MILP & 310.3 & 352.1 & 352.1 & 0.6 & 0.0 \\
c208 & 0 & 332.6 & 352.1 & 352.1 & 1.3 & 40.6 \\
c208 & 2 & 349.1 & 352.1 & 352.1 & 0.2 & 6.3 \\
c208 & 4 & 349.1 & 352.1 & 352.1 & 0.2 & 8.5 \\
c208 & 6 & 348.9 & 352.1 & 352.1 & 0.5 & 9.1 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_la_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_r100.tex <==
\begin{table}
\centering
\caption{Improvment via LA Choice:   Num Customers = 50 Problem Set = r100}
\label{tabLA:50Problem Set=r100}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time   \\
\midrule
r101 & BASELINE MILP & 1032.4 & 1046.7 & 1046.7 & 0.0 & 0.0 \\
r101 & 0 & 1046.7 & 1046.7 & 1046.7 & 0.0 & 0.1 \\
r101 & 2 & 1046.7 & 1046.7 & 1046.7 & 0.0 & 0.1 \\
r101 & 4 & 1046.7 & 1046.7 & 1046.7 & 0.0 & 0.1 \\
r101 & 6 & 1046.7 & 1046.7 & 1046.7 & 0.0 & 0.1 \\
r102 & BASELINE MILP & 651.9 & 911.4 & 911.4 & 51.1 & 0.0 \\
r102 & 0 & 911.4 & 911.4 & 911.4 & 0.2 & 0.8 \\
r102 & 2 & 911.4 & 911.4 & 911.4 & 0.2 & 1.1 \\
r102 & 4 & 911.4 & 911.4 & 911.4 & 0.1 & 1.1 \\
r102 & 6 & 911.4 & 911.4 & 911.4 & 0.1 & 1.5 \\
r103 & BASELINE MILP & 535.8 & 725.8 & 776.4 & 1000.0 & 0.0 \\
r103 & 0 & 758.9 & 775.7 & 775.7 & 3.8 & 14.7 \\
r103 & 2 & 765.0 & 775.6 & 775.7 & 1.4 & 14.7 \\
r103 & 4 & 765.0 & 775.7 & 775.7 & 3.1 & 11.5 \\
r103 & 6 & 765.0 & 775.7 & 775.7 & 2.2 & 10.8 \\
r104 & BASELINE MILP & 467.3 & 545.0 & 653.0 & 1000.1 & 0.0 \\
r104 & 0 & 611.1 & 631.3 & 631.3 & 51.2 & 63.1 \\
r104 & 2 & 614.6 & 631.3 & 631.3 & 55.5 & 66.0 \\
r104 & 4 & 614.6 & 631.3 & 631.3 & 58.9 & 71.4 \\
r104 & 6 & 614.6 & 631.3 & 631.3 & 52.6 & 75.4 \\
r105 & BASELINE MILP & 795.4 & 914.3 & 914.3 & 0.8 & 0.0 \\
r105 & 0 & 899.0 & 914.3 & 914.3 & 0.3 & 0.7 \\
r105 & 2 & 900.9 & 914.3 & 914.3 & 0.2 & 0.9 \\
r105 & 4 & 900.9 & 914.2 & 914.3 & 0.4 & 0.7 \\
r105 & 6 & 900.9 & 914.3 & 914.3 & 0.3 & 0.8 \\
r106 & BASELINE MILP & 549.4 & 795.3 & 795.3 & 629.0 & 0.0 \\
r106 & 0 & 793.0 & 795.3 & 795.3 & 0.2 & 3.1 \\
r106 & 2 & 794.9 & 795.3 & 795.3 & 0.2 & 3.2 \\
r106 & 4 & 794.9 & 795.3 & 795.3 & 0.2 & 3.8 \\
r106 & 6 & 794.9 & 795.3 & 795.3 & 0.2 & 4.1 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_la_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_r100pt2.tex <==
\begin{table}
\centering
\caption{Improvment via LA Choice:   Num Customers = 50 Problem Set = r100pt2}
\label{tabLA:50Problem Set=r100pt2}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time   \\
\midrule
r107 & BASELINE MILP & 485.9 & 634.5 & 713.5 & 1000.0 & 0.0 \\
r107 & 0 & 700.3 & 713.5 & 713.5 & 4.0 & 16.4 \\
r107 & 2 & 703.0 & 713.5 & 713.5 & 3.8 & 24.2 \\
r107 & 4 & 703.0 & 713.5 & 713.5 & 3.0 & 19.3 \\
r107 & 6 & 703.0 & 713.5 & 713.5 & 2.3 & 30.5 \\
r108 & BASELINE MILP & 460.2 & 533.4 & 633.8 & 1000.0 & 0.0 \\
r108 & 0 & 581.9 & 604.9 & 620.3 & 1000.0 & 109.9 \\
r108 & 2 & 587.4 & 603.1 & 620.3 & 1000.0 & 116.9 \\
r108 & 4 & 587.2 & 608.6 & 620.3 & 1000.1 & 97.4 \\
r108 & 6 & 587.5 & 605.9 & 620.3 & 1000.0 & 105.9 \\
r109 & BASELINE MILP & 549.9 & 771.2 & 791.3 & 1000.0 & 0.0 \\
r109 & 0 & 730.0 & 791.3 & 791.3 & 23.7 & 14.5 \\
r109 & 2 & 747.2 & 791.3 & 791.3 & 18.2 & 18.8 \\
r109 & 4 & 751.8 & 791.3 & 791.3 & 22.1 & 19.0 \\
r109 & 6 & 754.7 & 791.3 & 791.3 & 13.7 & 38.0 \\
r110 & BASELINE MILP & 483.2 & 613.5 & 699.4 & 1000.0 & 0.0 \\
r110 & 0 & 678.5 & 699.4 & 699.4 & 10.9 & 26.1 \\
r110 & 2 & 683.4 & 699.4 & 699.4 & 9.6 & 53.5 \\
r110 & 4 & 683.5 & 699.4 & 699.4 & 10.4 & 52.7 \\
r110 & 6 & 683.4 & 699.4 & 699.4 & 13.3 & 36.4 \\
r111 & BASELINE MILP & 478.0 & 607.6 & 711.0 & 1000.0 & 0.0 \\
r111 & 0 & 663.4 & 709.5 & 709.5 & 54.0 & 27.7 \\
r111 & 2 & 675.0 & 709.5 & 709.5 & 29.9 & 50.5 \\
r111 & 4 & 676.2 & 709.5 & 709.5 & 22.4 & 35.5 \\
r111 & 6 & 676.6 & 709.5 & 709.5 & 22.4 & 37.7 \\
r112 & BASELINE MILP & 454.5 & 520.1 & 654.6 & 1000.0 & 0.0 \\
r112 & 0 & 586.3 & 612.7 & 632.7 & 1000.0 & 90.3 \\
r112 & 2 & 596.6 & 624.5 & 632.7 & 1000.0 & 116.6 \\
r112 & 4 & 596.7 & 616.9 & 637.5 & 1000.0 & 136.2 \\
r112 & 6 & 596.5 & 617.8 & 632.7 & 1000.0 & 165.9 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_la_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_r200.tex <==
\begin{table}
\centering
\caption{Improvment via LA Choice:   Num Customers = 50 Problem Set = r200}
\label{tabLA:50Problem Set=r200}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time   \\
\midrule
r201 & BASELINE MILP & 703.1 & 794.3 & 794.3 & 0.2 & 0.0 \\
r201 & 0 & 756.3 & 794.3 & 794.3 & 0.3 & 4.3 \\
r201 & 2 & 788.1 & 794.3 & 794.3 & 0.2 & 2.5 \\
r201 & 4 & 791.4 & 794.3 & 794.3 & 0.4 & 3.7 \\
r201 & 6 & 791.7 & 794.3 & 794.3 & 0.1 & 3.1 \\
r202 & BASELINE MILP & 506.5 & 684.8 & 700.7 & 1000.0 & 0.0 \\
r202 & 0 & 640.3 & 700.7 & 700.7 & 7.4 & 27.4 \\
r202 & 2 & 682.0 & 700.7 & 700.7 & 2.2 & 50.8 \\
r202 & 4 & 682.5 & 700.7 & 700.7 & 3.1 & 48.0 \\
r202 & 6 & 682.6 & 700.7 & 700.7 & 4.8 & 76.7 \\
r203 & BASELINE MILP & 450.5 & 539.3 & 607.6 & 1000.0 & 0.0 \\
r203 & 0 & 541.0 & 607.6 & 607.6 & 102.3 & 47.9 \\
r203 & 2 & 568.3 & 607.6 & 607.6 & 82.1 & 55.1 \\
r203 & 4 & 571.4 & 607.6 & 607.6 & 47.2 & 72.2 \\
r203 & 6 & 572.6 & 607.6 & 607.6 & 51.8 & 178.7 \\
r204 & BASELINE MILP & 422.9 & 478.0 & 511.2 & 1000.0 & 0.0 \\
r204 & 0 & 442.5 & 481.5 & 511.2 & 1000.0 & 135.3 \\
r204 & 2 & 465.7 & 482.6 & 511.3 & 1000.0 & 254.6 \\
r204 & 4 & 465.9 & 487.5 & 510.6 & 1000.0 & 261.3 \\
r204 & 6 & 466.7 & 488.0 & 510.6 & 1000.0 & 246.7 \\
r205 & BASELINE MILP & 543.2 & 692.4 & 692.4 & 73.6 & 0.0 \\
r205 & 0 & 596.7 & 692.4 & 692.4 & 44.3 & 33.7 \\
r205 & 2 & 646.5 & 692.4 & 692.4 & 21.1 & 31.2 \\
r205 & 4 & 656.6 & 692.4 & 692.4 & 8.4 & 58.4 \\
r205 & 6 & 664.3 & 692.4 & 692.4 & 5.3 & 70.1 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_la_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_r200pt2.tex <==
\begin{table}
\centering
\caption{Improvment via LA Choice:   Num Customers = 50 Problem Set = r200pt2}
\label{tabLA:50Problem Set=r200pt2}
\begin{tabular}{ccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time   \\
\midrule
r206 & BASELINE MILP & 457.6 & 588.0 & 648.8 & 1000.0 & 0.0 \\
r206 & 0 & 533.6 & 629.8 & 634.9 & 1000.0 & 102.6 \\
r206 & 2 & 578.7 & 634.9 & 634.9 & 565.4 & 109.9 \\
r206 & 4 & 582.5 & 634.9 & 634.9 & 360.1 & 104.7 \\
r206 & 6 & 586.6 & 634.9 & 634.9 & 513.4 & 220.2 \\
r207 & BASELINE MILP & 423.3 & 521.9 & 601.8 & 1000.0 & 0.0 \\
r207 & 0 & 469.0 & 541.1 & 586.9 & 1000.1 & 170.5 \\
r207 & 2 & 514.3 & 551.9 & 578.7 & 1000.0 & 250.8 \\
r207 & 4 & 520.5 & 556.9 & 580.5 & 1000.1 & 182.1 \\
r207 & 6 & 522.1 & 559.5 & 577.7 & 1000.1 & 368.7 \\
r208 & BASELINE MILP & 414.7 & 471.9 & 505.0 & 1000.1 & 0.0 \\
r208 & 0 & 423.5 & 469.1 & 496.7 & 1000.0 & 226.1 \\
r208 & 2 & 457.1 & 473.3 & 490.0 & 1000.0 & 54.3 \\
r208 & 4 & 456.9 & 471.3 & 496.8 & 1000.0 & 53.9 \\
r208 & 6 & 457.4 & 470.9 & 494.8 & 1000.0 & 73.4 \\
r209 & BASELINE MILP & 483.7 & 603.1 & 603.1 & 373.7 & 0.0 \\
r209 & 0 & 537.7 & 603.1 & 603.1 & 261.9 & 98.0 \\
r209 & 2 & 567.8 & 603.1 & 603.1 & 115.8 & 111.4 \\
r209 & 4 & 570.7 & 603.1 & 603.1 & 71.6 & 110.3 \\
r209 & 6 & 571.1 & 603.1 & 603.1 & 94.3 & 139.8 \\
r210 & BASELINE MILP & 458.5 & 600.8 & 649.9 & 1000.0 & 0.0 \\
r210 & 0 & 534.3 & 633.7 & 647.9 & 1000.0 & 82.8 \\
r210 & 2 & 591.2 & 636.6 & 647.9 & 1000.0 & 97.2 \\
r210 & 4 & 595.0 & 647.9 & 647.9 & 922.4 & 111.8 \\
r210 & 6 & 595.7 & 647.9 & 647.9 & 823.5 & 171.3 \\
r211 & BASELINE MILP & 414.7 & 481.8 & 549.4 & 1000.0 & 0.0 \\
r211 & 0 & 459.9 & 502.2 & 559.5 & 1000.0 & 221.2 \\
r211 & 2 & 487.8 & 493.2 & 556.6 & 1000.0 & 626.4 \\
r211 & 4 & 489.3 & 505.2 & 538.0 & 1000.0 & 582.2 \\
r211 & 6 & 492.0 & 511.3 & 538.0 & 1000.0 & 501.1 \\
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_la_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_rc100.tex <==
\begin{table}
\centering
\caption{Improvment via LA Choice:   Num Customers = 50 Problem Set = rc100}
\label{tabLA:50Problem Set=rc100}
\begin{tabular}{}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time   \\
\midrule
\bottomrule
\end{tabular}
\end{table}

==> bene_results/bene_la_lat_ROUNDED_ALL_RESULTS_Num_Cust=50_rc200.tex <==
\begin{table}
\centering
\caption{Improvment via LA Choice:   Num Customers = 50 Problem Set = rc200}
\label{tabLA:50Problem Set=rc200}
\begin{tabular}{}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time   \\
\midrule
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=100_c100.tex <==
\begin{table}
\centering
\caption{Num Customers = 100 Problem Set = c100}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
c101 & OUR APPROACH & 827.3 & 827.3 & 827.3 & 0.2 & 2.9 &   \\
c101 & BASELINE MILP & 819.7 & 827.3 & 827.3 & 0.1 & 0.1 &   \\
c102 & OUR APPROACH & 827.1 & 827.3 & 827.3 & 1.8 & 47.7 &   \\
c102 & BASELINE MILP & 754.3 & 827.3 & 827.3 & 24.1 & 0.0 &   \\
c103 & OUR APPROACH & 826.1 & 826.3 & 826.3 & 19.0 & 136.8 & **** \\
c103 & BASELINE MILP & 588.9 & 785.0 & 826.3 & 1000.0 & 0.1 & **** \\
c104 & OUR APPROACH & 818.2 & 822.9 & 822.9 & 195.5 & 170.5 & **** \\
c104 & BASELINE MILP & 577.2 & 673.3 & 830.1 & 1000.0 & 0.1 & **** \\
c105 & OUR APPROACH & 827.3 & 827.3 & 827.3 & 0.3 & 3.2 &   \\
c105 & BASELINE MILP & 818.2 & 827.3 & 827.3 & 0.1 & 0.0 &   \\
c106 & OUR APPROACH & 827.3 & 827.3 & 827.3 & 0.4 & 10.9 &   \\
c106 & BASELINE MILP & 699.7 & 827.3 & 827.3 & 0.7 & 0.0 &   \\
c107 & OUR APPROACH & 827.3 & 827.3 & 827.3 & 0.5 & 5.9 &   \\
c107 & BASELINE MILP & 818.1 & 827.3 & 827.3 & 0.4 & 0.0 &   \\
c108 & OUR APPROACH & 827.3 & 827.3 & 827.3 & 5.0 & 71.2 &   \\
c108 & BASELINE MILP & 569.5 & 827.3 & 827.3 & 8.4 & 0.0 &   \\
c109 & OUR APPROACH & 825.1 & 827.3 & 827.3 & 54.8 & 145.2 & **** \\
c109 & BASELINE MILP & 566.0 & 792.1 & 853.4 & 1000.0 & 0.1 & **** \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=100_c200.tex <==
\begin{table}
\centering
\caption{Num Customers = 100 Problem Set = c200}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
c201 & OUR APPROACH & 589.1 & 589.1 & 589.1 & 0.1 & 5.5 &   \\
c201 & BASELINE MILP & 589.1 & 589.1 & 589.1 & 0.1 & 0.0 &   \\
c202 & OUR APPROACH & 589.1 & 589.1 & 589.1 & 0.3 & 65.6 &   \\
c202 & BASELINE MILP & 556.7 & 589.1 & 589.1 & 1.6 & 0.1 &   \\
c203 & OUR APPROACH & 583.7 & 588.7 & 588.7 & 13.9 & 127.4 &   \\
c203 & BASELINE MILP & 534.9 & 588.7 & 588.7 & 6.0 & 0.1 &   \\
c204 & OUR APPROACH & 582.4 & 588.1 & 588.1 & 61.6 & 183.7 &   \\
c204 & BASELINE MILP & 517.5 & 588.1 & 588.1 & 77.8 & 0.1 &   \\
c205 & OUR APPROACH & 586.0 & 586.4 & 586.4 & 0.3 & 29.5 &   \\
c205 & BASELINE MILP & 539.7 & 586.4 & 586.4 & 0.4 & 0.0 &   \\
c206 & OUR APPROACH & 586.0 & 586.0 & 586.0 & 0.2 & 33.1 &   \\
c206 & BASELINE MILP & 536.3 & 586.0 & 586.0 & 2.1 & 0.0 &   \\
c207 & OUR APPROACH & 582.7 & 585.8 & 585.8 & 5.2 & 98.5 &   \\
c207 & BASELINE MILP & 535.7 & 585.8 & 585.8 & 2.0 & 0.0 &   \\
c208 & OUR APPROACH & 583.4 & 585.8 & 585.8 & 1.0 & 72.0 &   \\
c208 & BASELINE MILP & 531.9 & 585.8 & 585.8 & 3.3 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=100_r100.tex <==
\begin{table}
\centering
\caption{Num Customers = 100 Problem Set = r100}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
r101 & OUR APPROACH & 1631.2 & 1637.7 & 1637.7 & 0.3 & 1.1 &   \\
r101 & BASELINE MILP & 1612.2 & 1637.7 & 1637.7 & 0.1 & 0.0 &   \\
r102 & OUR APPROACH & 1467.7 & 1467.7 & 1467.7 & 1.0 & 10.3 & **** \\
r102 & BASELINE MILP & 1027.2 & 1320.4 & 1470.5 & 1000.0 & 0.0 & **** \\
r103 & OUR APPROACH & 1204.2 & 1208.7 & 1208.7 & 9.1 & 65.6 & **** \\
r103 & BASELINE MILP & 787.2 & 999.1 & 1244.2 & 1000.0 & 0.1 & **** \\
r104 & OUR APPROACH & 944.9 & 946.5 & 1060.0 & 1000.0 & 338.2 &   \\
r104 & BASELINE MILP & 693.1 & 780.2 & 1012.8 & 1000.0 & 0.1 &   \\
r105 & OUR APPROACH & 1341.6 & 1355.3 & 1355.3 & 5.6 & 24.0 & **** \\
r105 & BASELINE MILP & 1098.2 & 1355.3 & 1355.3 & 440.9 & 0.0 & **** \\
r106 & OUR APPROACH & 1215.4 & 1234.6 & 1234.6 & 70.2 & 95.6 & **** \\
r106 & BASELINE MILP & 833.3 & 1016.2 & 1266.9 & 1000.0 & 0.1 & **** \\
r107 & OUR APPROACH & 1040.6 & 1049.8 & 1070.6 & 1000.0 & 201.7 &   \\
r107 & BASELINE MILP & 719.2 & 827.8 & 1126.8 & 1000.1 & 0.1 &   \\
r108 & OUR APPROACH & 906.9 & 908.6 & 1151.9 & 999.9 & 411.1 &   \\
r108 & BASELINE MILP & 679.8 & 736.3 & 997.1 & 1000.0 & 0.1 &   \\
r109 & OUR APPROACH & 1109.3 & 1136.7 & 1146.9 & 1000.0 & 109.2 &   \\
r109 & BASELINE MILP & 775.6 & 939.7 & 1194.9 & 1000.0 & 0.0 &   \\
r110 & OUR APPROACH & 1028.8 & 1034.9 & 1078.8 & 1000.2 & 188.2 &   \\
r110 & BASELINE MILP & 704.3 & 794.3 & 1115.9 & 1000.0 & 0.1 &   \\
r111 & OUR APPROACH & 1012.7 & 1026.3 & 1050.6 & 1000.0 & 193.2 &   \\
r111 & BASELINE MILP & 704.0 & 803.5 & 1126.2 & 1000.0 & 0.1 &   \\
r112 & OUR APPROACH & 910.0 & 911.1 & 1070.6 & 1000.0 & 438.7 &   \\
r112 & BASELINE MILP & 668.9 & 716.6 & 1069.9 & 1000.1 & 0.1 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=100_r200.tex <==
\begin{table}
\centering
\caption{Num Customers = 100 Problem Set = r200}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
r201 & OUR APPROACH & 1114.0 & 1143.2 & 1143.2 & 5.0 & 119.5 &   \\
r201 & BASELINE MILP & 979.2 & 1143.2 & 1143.2 & 21.2 & 0.0 &   \\
r202 & OUR APPROACH & 974.2 & 1006.9 & 1029.6 & 1000.0 & 362.9 &   \\
r202 & BASELINE MILP & 731.0 & 872.7 & 1049.5 & 1000.0 & 0.0 &   \\
r203 & OUR APPROACH & 794.0 & 809.0 & 883.2 & 1000.0 & 636.0 &   \\
r203 & BASELINE MILP & 633.0 & 716.7 & 906.3 & 1000.0 & 0.1 &   \\
r204 & OUR APPROACH & 668.0 & 675.8 & 770.1 & 1000.0 & 804.5 &   \\
r204 & BASELINE MILP & 591.1 & 647.9 & 789.8 & 1000.1 & 0.1 &   \\
r205 & OUR APPROACH & 891.0 & 912.4 & 954.7 & 1000.0 & 473.6 &   \\
r205 & BASELINE MILP & 738.1 & 879.8 & 967.4 & 1000.0 & 0.0 &   \\
r206 & OUR APPROACH & 803.7 & 825.6 & 898.0 & 1000.0 & 798.7 &   \\
r206 & BASELINE MILP & 651.9 & 758.2 & 914.6 & 1000.0 & 0.1 &   \\
r207 & OUR APPROACH & 719.4 & 728.3 & 900.0 & 1000.0 & 1687.1 &   \\
r207 & BASELINE MILP & 612.2 & 691.4 & 815.7 & 1000.1 & 0.1 &   \\
r208 & OUR APPROACH & 643.2 & 645.4 & 823.4 & 1000.0 & 396.1 &   \\
r208 & BASELINE MILP & 583.6 & 643.7 & 729.6 & 1000.0 & 0.1 &   \\
r209 & OUR APPROACH & 790.8 & 804.2 & 905.7 & 1000.0 & 339.0 &   \\
r209 & BASELINE MILP & 653.0 & 758.1 & 859.2 & 1000.0 & 0.1 &   \\
r210 & OUR APPROACH & 808.6 & 826.3 & 934.0 & 1000.0 & 407.7 &   \\
r210 & BASELINE MILP & 644.9 & 760.2 & 928.6 & 1000.0 & 0.1 &   \\
r211 & OUR APPROACH & 667.5 & 672.0 & 881.2 & 1000.0 & 292.8 &   \\
r211 & BASELINE MILP & 583.6 & 642.3 & 799.2 & 1000.1 & 0.1 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=100_rc100.tex <==
\begin{table}
\centering
\caption{Num Customers = 100 Problem Set = rc100}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
rc101 & OUR APPROACH & 1577.3 & 1619.8 & 1619.8 & 17.8 & 28.8 &   \\
rc101 & BASELINE MILP & 1131.3 & 1619.8 & 1619.8 & 316.1 & 0.1 &   \\
rc102 & OUR APPROACH & 1384.2 & 1431.9 & 1457.4 & 1000.1 & 126.4 &   \\
rc102 & BASELINE MILP & 795.6 & 1098.7 & 1481.6 & 1000.0 & 0.0 &   \\
rc103 & OUR APPROACH & 1176.8 & 1185.9 & 1288.1 & 1000.0 & 320.6 &   \\
rc103 & BASELINE MILP & 694.5 & 857.3 & 1389.1 & 1000.1 & 0.1 &   \\
rc104 & OUR APPROACH & 1050.6 & 1060.8 & 1227.4 & 1000.0 & 327.8 &   \\
rc104 & BASELINE MILP & 670.4 & 782.6 & 1197.0 & 1000.1 & 0.1 &   \\
rc105 & OUR APPROACH & 1461.4 & 1513.7 & 1513.7 & 94.9 & 52.3 & **** \\
rc105 & BASELINE MILP & 927.5 & 1268.4 & 1552.8 & 1000.0 & 0.0 & **** \\
rc106 & OUR APPROACH & 1269.2 & 1294.2 & 1373.5 & 1000.1 & 133.0 &   \\
rc106 & BASELINE MILP & 782.3 & 1018.0 & 1411.6 & 1000.1 & 0.0 &   \\
rc107 & OUR APPROACH & 1125.0 & 1139.8 & 1260.9 & 1000.1 & 333.8 &   \\
rc107 & BASELINE MILP & 681.9 & 803.0 & 1358.8 & 1000.1 & 0.1 &   \\
rc108 & OUR APPROACH & 1041.3 & 1047.3 & 1235.9 & 1000.1 & 319.9 &   \\
rc108 & BASELINE MILP & 663.1 & 738.0 & 1217.6 & 999.4 & 0.1 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=100_rc200.tex <==
\begin{table}
\centering
\caption{Num Customers = 100 Problem Set = rc200}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
rc201 & OUR APPROACH & 1214.0 & 1261.8 & 1261.8 & 6.8 & 90.1 &   \\
rc201 & BASELINE MILP & 946.2 & 1261.8 & 1261.8 & 119.0 & 0.0 &   \\
rc202 & OUR APPROACH & 963.6 & 1008.1 & 1100.7 & 1000.4 & 428.7 &   \\
rc202 & BASELINE MILP & 659.9 & 863.3 & 1124.3 & 1000.0 & 0.0 &   \\
rc203 & OUR APPROACH & 764.0 & 779.5 & 1088.5 & 1000.0 & 305.4 &   \\
rc203 & BASELINE MILP & 575.8 & 702.1 & 976.7 & 1000.1 & 0.1 &   \\
rc204 & OUR APPROACH & 647.3 & 655.4 & 943.0 & 1000.1 & 312.3 &   \\
rc204 & BASELINE MILP & 544.5 & 628.9 & 812.4 & 1000.0 & 0.1 &   \\
rc205 & OUR APPROACH & 1045.5 & 1083.8 & 1159.2 & 1000.0 & 317.5 &   \\
rc205 & BASELINE MILP & 759.1 & 1029.0 & 1178.1 & 1000.0 & 0.0 &   \\
rc206 & OUR APPROACH & 951.1 & 969.7 & 1058.1 & 1000.0 & 414.7 &   \\
rc206 & BASELINE MILP & 710.3 & 905.4 & 1066.7 & 1000.0 & 0.0 &   \\
rc207 & OUR APPROACH & 841.5 & 857.2 & 1060.3 & 1000.0 & 309.2 &   \\
rc207 & BASELINE MILP & 602.0 & 738.3 & 988.1 & 1000.0 & 0.1 &   \\
rc208 & OUR APPROACH & 646.0 & 652.6 & 995.3 & 1000.0 & 324.3 &   \\
rc208 & BASELINE MILP & 536.8 & 609.2 & 854.5 & 1000.0 & 0.1 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=25_c100.tex <==
\begin{table}
\centering
\caption{Num Customers = 25 Problem Set = c100}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
c101 & OUR APPROACH & 191.3 & 191.3 & 191.3 & 0.0 & 0.1 &   \\
c101 & BASELINE MILP & 191.3 & 191.3 & 191.3 & 0.0 & 0.0 &   \\
c102 & OUR APPROACH & 190.3 & 190.3 & 190.3 & 0.0 & 0.4 &   \\
c102 & BASELINE MILP & 172.7 & 190.3 & 190.3 & 0.2 & 0.0 &   \\
c103 & OUR APPROACH & 190.3 & 190.3 & 190.3 & 0.1 & 2.0 &   \\
c103 & BASELINE MILP & 163.8 & 190.3 & 190.3 & 0.6 & 0.0 &   \\
c104 & OUR APPROACH & 186.9 & 186.9 & 186.9 & 0.1 & 2.8 &   \\
c104 & BASELINE MILP & 160.5 & 186.9 & 186.9 & 2.4 & 0.0 &   \\
c105 & OUR APPROACH & 191.3 & 191.3 & 191.3 & 0.0 & 0.1 &   \\
c105 & BASELINE MILP & 191.2 & 191.3 & 191.3 & 0.0 & 0.0 &   \\
c106 & OUR APPROACH & 191.3 & 191.3 & 191.3 & 0.0 & 0.1 &   \\
c106 & BASELINE MILP & 191.3 & 191.3 & 191.3 & 0.0 & 0.0 &   \\
c107 & OUR APPROACH & 191.3 & 191.3 & 191.3 & 0.0 & 0.1 &   \\
c107 & BASELINE MILP & 191.2 & 191.3 & 191.3 & 0.0 & 0.0 &   \\
c108 & OUR APPROACH & 191.3 & 191.3 & 191.3 & 0.0 & 1.1 &   \\
c108 & BASELINE MILP & 131.5 & 191.3 & 191.3 & 0.2 & 0.0 &   \\
c109 & OUR APPROACH & 190.6 & 191.3 & 191.3 & 0.2 & 6.4 &   \\
c109 & BASELINE MILP & 131.1 & 191.3 & 191.3 & 0.8 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=25_c200.tex <==
\begin{table}
\centering
\caption{Num Customers = 25 Problem Set = c200}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
c201 & OUR APPROACH & 214.7 & 214.7 & 214.7 & 0.0 & 0.1 &   \\
c201 & BASELINE MILP & 214.7 & 214.7 & 214.7 & 0.0 & 0.0 &   \\
c202 & OUR APPROACH & 214.7 & 214.7 & 214.7 & 0.0 & 2.0 &   \\
c202 & BASELINE MILP & 175.0 & 214.7 & 214.7 & 0.6 & 0.0 &   \\
c203 & OUR APPROACH & 214.7 & 214.7 & 214.7 & 0.0 & 3.3 &   \\
c203 & BASELINE MILP & 169.5 & 214.7 & 214.7 & 1.5 & 0.0 &   \\
c204 & OUR APPROACH & 209.6 & 213.1 & 213.1 & 1.0 & 8.6 &   \\
c204 & BASELINE MILP & 165.4 & 213.1 & 213.1 & 24.9 & 0.0 &   \\
c205 & OUR APPROACH & 214.7 & 214.7 & 214.7 & 0.0 & 0.3 &   \\
c205 & BASELINE MILP & 176.4 & 214.7 & 214.7 & 0.0 & 0.0 &   \\
c206 & OUR APPROACH & 214.7 & 214.7 & 214.7 & 0.0 & 0.5 &   \\
c206 & BASELINE MILP & 173.1 & 214.7 & 214.7 & 0.2 & 0.0 &   \\
c207 & OUR APPROACH & 211.3 & 214.5 & 214.5 & 0.2 & 5.8 &   \\
c207 & BASELINE MILP & 166.7 & 214.5 & 214.5 & 1.0 & 0.0 &   \\
c208 & OUR APPROACH & 211.7 & 214.5 & 214.5 & 0.1 & 1.1 &   \\
c208 & BASELINE MILP & 166.4 & 214.5 & 214.5 & 0.3 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=25_r100.tex <==
\begin{table}
\centering
\caption{Num Customers = 25 Problem Set = r100}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
r101 & OUR APPROACH & 617.1 & 617.1 & 617.1 & 0.0 & 0.0 &   \\
r101 & BASELINE MILP & 617.1 & 617.1 & 617.1 & 0.0 & 0.0 &   \\
r102 & OUR APPROACH & 546.3 & 547.1 & 547.1 & 0.0 & 0.1 &   \\
r102 & BASELINE MILP & 384.7 & 547.1 & 547.1 & 0.4 & 0.0 &   \\
r103 & OUR APPROACH & 454.2 & 454.6 & 454.6 & 0.1 & 0.9 &   \\
r103 & BASELINE MILP & 328.9 & 454.6 & 454.6 & 3.9 & 0.0 &   \\
r104 & OUR APPROACH & 415.0 & 416.9 & 416.9 & 0.1 & 1.4 & **** \\
r104 & BASELINE MILP & 319.5 & 416.9 & 416.9 & 36.2 & 0.0 & **** \\
r105 & OUR APPROACH & 530.5 & 530.5 & 530.5 & 0.0 & 0.0 &   \\
r105 & BASELINE MILP & 456.5 & 530.5 & 530.5 & 0.1 & 0.0 &   \\
r106 & OUR APPROACH & 457.3 & 465.4 & 465.4 & 0.1 & 0.3 &   \\
r106 & BASELINE MILP & 346.3 & 465.4 & 465.4 & 0.6 & 0.0 &   \\
r107 & OUR APPROACH & 417.4 & 424.3 & 424.3 & 0.1 & 1.8 &   \\
r107 & BASELINE MILP & 319.7 & 424.3 & 424.3 & 6.8 & 0.0 &   \\
r108 & OUR APPROACH & 391.7 & 397.3 & 397.3 & 0.2 & 5.5 &   \\
r108 & BASELINE MILP & 311.0 & 397.3 & 397.3 & 20.4 & 0.0 &   \\
r109 & OUR APPROACH & 440.3 & 441.3 & 441.3 & 0.1 & 0.4 &   \\
r109 & BASELINE MILP & 347.3 & 441.3 & 441.3 & 0.2 & 0.0 &   \\
r110 & OUR APPROACH & 421.5 & 444.1 & 444.1 & 1.0 & 2.7 & **** \\
r110 & BASELINE MILP & 312.8 & 444.1 & 444.1 & 65.8 & 0.0 & **** \\
r111 & OUR APPROACH & 418.4 & 428.8 & 428.8 & 0.2 & 1.8 &   \\
r111 & BASELINE MILP & 320.6 & 428.8 & 428.8 & 5.3 & 0.0 &   \\
r112 & OUR APPROACH & 371.3 & 393.0 & 393.0 & 2.2 & 9.7 & **** \\
r112 & BASELINE MILP & 309.9 & 393.0 & 393.0 & 353.0 & 0.0 & **** \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=25_r200.tex <==
\begin{table}
\centering
\caption{Num Customers = 25 Problem Set = r200}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
r201 & OUR APPROACH & 458.6 & 463.3 & 463.3 & 0.0 & 0.4 &   \\
r201 & BASELINE MILP & 417.0 & 463.3 & 463.3 & 0.0 & 0.0 &   \\
r202 & OUR APPROACH & 399.6 & 410.5 & 410.5 & 0.2 & 2.0 &   \\
r202 & BASELINE MILP & 314.7 & 410.5 & 410.5 & 1.5 & 0.0 &   \\
r203 & OUR APPROACH & 362.5 & 391.4 & 391.4 & 0.9 & 8.8 &   \\
r203 & BASELINE MILP & 302.3 & 391.4 & 391.4 & 43.0 & 0.0 &   \\
r204 & OUR APPROACH & 322.2 & 355.0 & 355.0 & 2.5 & 15.7 &   \\
r204 & BASELINE MILP & 292.6 & 355.0 & 355.0 & 29.6 & 0.0 &   \\
r205 & OUR APPROACH & 386.4 & 393.0 & 393.0 & 0.1 & 2.4 &   \\
r205 & BASELINE MILP & 337.9 & 393.0 & 393.0 & 0.6 & 0.0 &   \\
r206 & OUR APPROACH & 349.2 & 374.4 & 374.4 & 1.7 & 11.3 &   \\
r206 & BASELINE MILP & 292.9 & 374.4 & 374.4 & 5.1 & 0.0 &   \\
r207 & OUR APPROACH & 338.4 & 361.6 & 361.6 & 2.9 & 23.3 &   \\
r207 & BASELINE MILP & 292.4 & 361.6 & 361.6 & 11.2 & 0.0 &   \\
r208 & OUR APPROACH & 312.3 & 328.2 & 328.2 & 2.0 & 8.1 &   \\
r208 & BASELINE MILP & 292.3 & 328.2 & 328.2 & 2.9 & 0.0 &   \\
r209 & OUR APPROACH & 354.6 & 370.7 & 370.7 & 0.9 & 5.3 &   \\
r209 & BASELINE MILP & 303.3 & 370.7 & 370.7 & 0.8 & 0.0 &   \\
r210 & OUR APPROACH & 378.3 & 404.6 & 404.6 & 1.9 & 9.5 &   \\
r210 & BASELINE MILP & 302.7 & 404.6 & 404.6 & 1.8 & 0.0 &   \\
r211 & OUR APPROACH & 313.6 & 350.9 & 350.9 & 19.2 & 19.1 &   \\
r211 & BASELINE MILP & 292.4 & 350.9 & 350.9 & 44.7 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=25_rc100.tex <==
\begin{table}
\centering
\caption{Num Customers = 25 Problem Set = rc100}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
rc101 & OUR APPROACH & 402.8 & 461.1 & 461.1 & 0.1 & 0.3 &   \\
rc101 & BASELINE MILP & 336.3 & 461.1 & 461.1 & 0.1 & 0.0 &   \\
rc102 & OUR APPROACH & 350.9 & 351.8 & 351.8 & 0.1 & 0.7 &   \\
rc102 & BASELINE MILP & 302.5 & 351.8 & 351.8 & 0.4 & 0.0 &   \\
rc103 & OUR APPROACH & 319.2 & 332.8 & 332.8 & 0.4 & 3.1 &   \\
rc103 & BASELINE MILP & 280.9 & 332.8 & 332.8 & 9.5 & 0.0 &   \\
rc104 & OUR APPROACH & 302.0 & 306.6 & 306.6 & 0.3 & 2.1 &   \\
rc104 & BASELINE MILP & 278.9 & 306.6 & 306.6 & 1.5 & 0.0 &   \\
rc105 & OUR APPROACH & 408.5 & 411.3 & 411.3 & 0.1 & 0.6 &   \\
rc105 & BASELINE MILP & 308.0 & 411.3 & 411.3 & 4.4 & 0.0 &   \\
rc106 & OUR APPROACH & 334.7 & 345.5 & 345.5 & 0.5 & 4.7 &   \\
rc106 & BASELINE MILP & 299.0 & 345.5 & 345.5 & 0.7 & 0.0 &   \\
rc107 & OUR APPROACH & 297.8 & 298.3 & 298.3 & 0.1 & 2.1 &   \\
rc107 & BASELINE MILP & 272.9 & 298.3 & 298.3 & 0.6 & 0.0 &   \\
rc108 & OUR APPROACH & 293.7 & 294.5 & 294.5 & 0.7 & 16.9 &   \\
rc108 & BASELINE MILP & 272.4 & 294.5 & 294.5 & 0.9 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=25_rc200.tex <==
\begin{table}
\centering
\caption{Num Customers = 25 Problem Set = rc200}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
rc201 & OUR APPROACH & 358.8 & 360.2 & 360.2 & 0.0 & 0.2 &   \\
rc201 & BASELINE MILP & 274.0 & 360.2 & 360.2 & 0.1 & 0.0 &   \\
rc202 & OUR APPROACH & 307.3 & 338.0 & 338.0 & 1.5 & 10.1 &   \\
rc202 & BASELINE MILP & 181.7 & 338.0 & 338.0 & 29.0 & 0.0 &   \\
rc203 & OUR APPROACH & 259.6 & 326.9 & 326.9 & 329.4 & 34.6 & **** \\
rc203 & BASELINE MILP & 162.6 & 245.7 & 326.9 & 1000.0 & 0.0 & **** \\
rc204 & OUR APPROACH & 238.0 & 269.0 & 299.7 & 1000.1 & 11.8 &   \\
rc204 & BASELINE MILP & 157.8 & 195.3 & 299.7 & 1000.0 & 0.0 &   \\
rc205 & OUR APPROACH & 314.1 & 338.0 & 338.0 & 0.1 & 1.1 &   \\
rc205 & BASELINE MILP & 193.7 & 338.0 & 338.0 & 0.4 & 0.0 &   \\
rc206 & OUR APPROACH & 301.3 & 324.0 & 324.0 & 0.6 & 2.8 &   \\
rc206 & BASELINE MILP & 183.2 & 324.0 & 324.0 & 1.7 & 0.0 &   \\
rc207 & OUR APPROACH & 254.5 & 298.3 & 298.3 & 34.8 & 14.4 & **** \\
rc207 & BASELINE MILP & 153.7 & 274.2 & 298.3 & 1000.0 & 0.0 & **** \\
rc208 & OUR APPROACH & 168.1 & 186.0 & 269.1 & 1000.0 & 17.4 &   \\
rc208 & BASELINE MILP & 148.3 & 190.0 & 269.1 & 1000.0 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=50_c100.tex <==
\begin{table}
\centering
\caption{Num Customers = 50 Problem Set = c100}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
c101 & OUR APPROACH & 362.4 & 362.4 & 362.4 & 0.1 & 0.5 &   \\
c101 & BASELINE MILP & 361.4 & 362.4 & 362.4 & 0.0 & 0.0 &   \\
c102 & OUR APPROACH & 361.4 & 361.4 & 361.4 & 0.2 & 2.4 &   \\
c102 & BASELINE MILP & 334.0 & 361.4 & 361.4 & 0.5 & 0.0 &   \\
c103 & OUR APPROACH & 361.4 & 361.4 & 361.4 & 0.8 & 40.3 &   \\
c103 & BASELINE MILP & 284.7 & 361.4 & 361.4 & 15.1 & 0.0 &   \\
c104 & OUR APPROACH & 355.2 & 358.0 & 358.0 & 11.9 & 118.5 & **** \\
c104 & BASELINE MILP & 281.0 & 312.4 & 358.0 & 1000.0 & 0.0 & **** \\
c105 & OUR APPROACH & 362.4 & 362.4 & 362.4 & 0.1 & 1.2 &   \\
c105 & BASELINE MILP & 360.0 & 362.4 & 362.4 & 0.1 & 0.0 &   \\
c106 & OUR APPROACH & 362.4 & 362.4 & 362.4 & 0.1 & 0.9 &   \\
c106 & BASELINE MILP & 360.1 & 362.4 & 362.4 & 0.1 & 0.0 &   \\
c107 & OUR APPROACH & 362.4 & 362.4 & 362.4 & 0.1 & 1.7 &   \\
c107 & BASELINE MILP & 360.0 & 362.4 & 362.4 & 0.1 & 0.0 &   \\
c108 & OUR APPROACH & 362.4 & 362.4 & 362.4 & 0.2 & 6.2 &   \\
c108 & BASELINE MILP & 261.1 & 362.4 & 362.4 & 0.9 & 0.0 &   \\
c109 & OUR APPROACH & 361.7 & 362.4 & 362.4 & 1.8 & 51.0 &   \\
c109 & BASELINE MILP & 257.1 & 362.4 & 362.4 & 16.1 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=50_c200.tex <==
\begin{table}
\centering
\caption{Num Customers = 50 Problem Set = c200}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
c201 & OUR APPROACH & 360.2 & 360.2 & 360.2 & 0.0 & 0.9 &   \\
c201 & BASELINE MILP & 360.2 & 360.2 & 360.2 & 0.0 & 0.0 &   \\
c202 & OUR APPROACH & 360.2 & 360.2 & 360.2 & 0.1 & 11.9 &   \\
c202 & BASELINE MILP & 318.2 & 360.2 & 360.2 & 2.0 & 0.0 &   \\
c203 & OUR APPROACH & 359.8 & 359.8 & 359.8 & 0.2 & 35.5 &   \\
c203 & BASELINE MILP & 299.1 & 359.8 & 359.8 & 22.5 & 0.0 &   \\
c204 & OUR APPROACH & 349.9 & 350.1 & 350.1 & 0.8 & 89.8 & **** \\
c204 & BASELINE MILP & 288.6 & 345.8 & 350.1 & 1000.0 & 0.0 & **** \\
c205 & OUR APPROACH & 359.8 & 359.8 & 359.8 & 0.1 & 2.5 &   \\
c205 & BASELINE MILP & 313.1 & 359.8 & 359.8 & 0.2 & 0.0 &   \\
c206 & OUR APPROACH & 359.8 & 359.8 & 359.8 & 0.1 & 4.4 &   \\
c206 & BASELINE MILP & 310.9 & 359.8 & 359.8 & 0.9 & 0.0 &   \\
c207 & OUR APPROACH & 356.5 & 359.6 & 359.6 & 1.8 & 49.4 &   \\
c207 & BASELINE MILP & 310.7 & 359.6 & 359.6 & 1.3 & 0.0 &   \\
c208 & OUR APPROACH & 347.4 & 350.5 & 350.5 & 0.2 & 7.7 &   \\
c208 & BASELINE MILP & 309.0 & 350.5 & 350.5 & 0.8 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=50_r100.tex <==
\begin{table}
\centering
\caption{Num Customers = 50 Problem Set = r100}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
r101 & OUR APPROACH & 1044.0 & 1044.0 & 1044.0 & 0.0 & 0.1 &   \\
r101 & BASELINE MILP & 1029.8 & 1044.0 & 1044.0 & 0.0 & 0.0 &   \\
r102 & OUR APPROACH & 909.0 & 909.0 & 909.0 & 0.1 & 1.2 & **** \\
r102 & BASELINE MILP & 649.7 & 909.0 & 909.0 & 54.9 & 0.0 & **** \\
r103 & OUR APPROACH & 762.1 & 772.9 & 772.9 & 3.1 & 12.7 & **** \\
r103 & BASELINE MILP & 533.1 & 721.7 & 772.9 & 1000.0 & 0.0 & **** \\
r104 & OUR APPROACH & 612.1 & 625.4 & 625.4 & 22.7 & 95.3 & **** \\
r104 & BASELINE MILP & 464.6 & 541.6 & 636.0 & 1000.0 & 0.0 & **** \\
r105 & OUR APPROACH & 898.5 & 911.8 & 911.8 & 0.3 & 0.8 &   \\
r105 & BASELINE MILP & 793.0 & 911.8 & 911.8 & 1.2 & 0.0 &   \\
r106 & OUR APPROACH & 792.7 & 793.0 & 793.0 & 0.3 & 4.1 & **** \\
r106 & BASELINE MILP & 547.0 & 793.0 & 793.0 & 561.0 & 0.0 & **** \\
r107 & OUR APPROACH & 700.5 & 711.1 & 711.1 & 4.4 & 37.1 & **** \\
r107 & BASELINE MILP & 483.2 & 631.7 & 724.4 & 1000.0 & 0.0 & **** \\
r108 & OUR APPROACH & 584.9 & 608.1 & 617.7 & 1000.0 & 160.2 &   \\
r108 & BASELINE MILP & 457.5 & 530.6 & 624.7 & 1000.0 & 0.0 &   \\
r109 & OUR APPROACH & 752.1 & 786.8 & 786.8 & 9.5 & 37.9 & **** \\
r109 & BASELINE MILP & 547.2 & 767.5 & 786.8 & 1000.0 & 0.0 & **** \\
r110 & OUR APPROACH & 681.1 & 697.0 & 697.0 & 9.9 & 68.5 & **** \\
r110 & BASELINE MILP & 481.0 & 606.3 & 713.0 & 1000.0 & 0.0 & **** \\
r111 & OUR APPROACH & 673.0 & 707.2 & 707.2 & 35.5 & 31.5 & **** \\
r111 & BASELINE MILP & 475.4 & 603.8 & 714.2 & 1000.0 & 0.0 & **** \\
r112 & OUR APPROACH & 593.3 & 613.9 & 630.2 & 1000.0 & 146.8 &   \\
r112 & BASELINE MILP & 451.8 & 513.2 & 647.9 & 1000.0 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=50_r200.tex <==
\begin{table}
\centering
\caption{Num Customers = 50 Problem Set = r200}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
r201 & OUR APPROACH & 789.5 & 791.9 & 791.9 & 0.1 & 3.5 &   \\
r201 & BASELINE MILP & 700.9 & 791.9 & 791.9 & 0.3 & 0.0 &   \\
r202 & OUR APPROACH & 680.5 & 698.5 & 698.5 & 6.6 & 39.4 & **** \\
r202 & BASELINE MILP & 504.4 & 682.4 & 698.5 & 1000.0 & 0.0 & **** \\
r203 & OUR APPROACH & 570.2 & 605.3 & 605.3 & 36.1 & 104.7 & **** \\
r203 & BASELINE MILP & 447.9 & 540.0 & 605.9 & 1000.0 & 0.0 & **** \\
r204 & OUR APPROACH & 464.6 & 487.8 & 508.1 & 1000.0 & 378.8 &   \\
r204 & BASELINE MILP & 420.4 & 477.4 & 508.9 & 1000.0 & 0.0 &   \\
r205 & OUR APPROACH & 662.2 & 690.1 & 690.1 & 6.7 & 65.9 &   \\
r205 & BASELINE MILP & 540.9 & 690.1 & 690.1 & 120.7 & 0.0 &   \\
r206 & OUR APPROACH & 584.4 & 632.4 & 632.4 & 445.2 & 141.4 & **** \\
r206 & BASELINE MILP & 455.2 & 581.8 & 639.0 & 1000.0 & 0.0 & **** \\
r207 & OUR APPROACH & 519.9 & 556.5 & 576.1 & 1000.0 & 438.9 &   \\
r207 & BASELINE MILP & 420.6 & 521.6 & 575.5 & 1000.0 & 0.0 &   \\
r208 & OUR APPROACH & 455.6 & 468.1 & 487.7 & 1000.0 & 118.7 &   \\
r208 & BASELINE MILP & 412.1 & 469.9 & 494.2 & 1000.0 & 0.0 &   \\
r209 & OUR APPROACH & 568.6 & 600.6 & 600.6 & 64.7 & 153.6 &   \\
r209 & BASELINE MILP & 481.2 & 600.6 & 600.6 & 287.4 & 0.0 &   \\
r210 & OUR APPROACH & 592.8 & 645.6 & 645.6 & 841.9 & 211.2 & **** \\
r210 & BASELINE MILP & 456.2 & 591.2 & 647.8 & 1000.0 & 0.0 & **** \\
r211 & OUR APPROACH & 489.8 & 504.6 & 540.9 & 1000.0 & 563.4 &   \\
r211 & BASELINE MILP & 412.1 & 479.3 & 541.3 & 1000.0 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=50_rc100.tex <==
\begin{table}
\centering
\caption{Num Customers = 50 Problem Set = rc100}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
rc101 & OUR APPROACH & 841.4 & 944.0 & 944.0 & 2.7 & 3.8 &   \\
rc101 & BASELINE MILP & 610.6 & 944.0 & 944.0 & 5.3 & 0.0 &   \\
rc102 & OUR APPROACH & 710.2 & 822.5 & 822.5 & 303.9 & 24.7 & **** \\
rc102 & BASELINE MILP & 515.9 & 751.5 & 822.5 & 1000.0 & 0.0 & **** \\
rc103 & OUR APPROACH & 623.0 & 672.2 & 710.9 & 1000.0 & 73.6 &   \\
rc103 & BASELINE MILP & 480.0 & 575.3 & 711.5 & 1000.0 & 0.0 &   \\
rc104 & OUR APPROACH & 529.8 & 545.8 & 545.8 & 56.9 & 208.9 & **** \\
rc104 & BASELINE MILP & 467.6 & 523.2 & 545.8 & 1000.0 & 0.0 & **** \\
rc105 & OUR APPROACH & 747.9 & 855.3 & 855.3 & 6.8 & 8.5 & **** \\
rc105 & BASELINE MILP & 533.6 & 791.8 & 855.3 & 1000.1 & 0.0 & **** \\
rc106 & OUR APPROACH & 648.5 & 723.2 & 723.2 & 27.1 & 69.7 & **** \\
rc106 & BASELINE MILP & 500.9 & 618.3 & 723.2 & 999.9 & 0.0 & **** \\
rc107 & OUR APPROACH & 573.3 & 642.7 & 642.7 & 616.1 & 157.3 & **** \\
rc107 & BASELINE MILP & 470.9 & 559.0 & 642.7 & 1000.0 & 0.0 & **** \\
rc108 & OUR APPROACH & 528.4 & 536.2 & 598.1 & 1000.0 & 208.0 &   \\
rc108 & BASELINE MILP & 463.2 & 502.7 & 599.4 & 1000.0 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> lat_ROUNDED_ALL_RESULTS_Num_Cust=50_rc200.tex <==
\begin{table}
\centering
\caption{Num Customers = 50 Problem Set = rc200}
\label{tab:example}
\begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\toprule
file num & Approach & lp obj & mip dual bound & ILP obj & ilp time & total lp time & 10X+  \\
\midrule
rc201 & OUR APPROACH & 677.9 & 684.8 & 684.8 & 0.2 & 2.0 &   \\
rc201 & BASELINE MILP & 385.5 & 684.8 & 684.8 & 0.8 & 0.0 &   \\
rc202 & OUR APPROACH & 539.8 & 613.6 & 613.6 & 591.1 & 180.3 & **** \\
rc202 & BASELINE MILP & 296.3 & 522.1 & 613.6 & 1000.0 & 0.0 & **** \\
rc203 & OUR APPROACH & 437.6 & 474.0 & 555.3 & 1000.0 & 463.5 &   \\
rc203 & BASELINE MILP & 257.3 & 365.2 & 557.3 & 1000.0 & 0.0 &   \\
rc204 & OUR APPROACH & 307.0 & 315.1 & 449.8 & 1000.0 & 1683.8 &   \\
rc204 & BASELINE MILP & 237.0 & 273.9 & 444.2 & 1000.0 & 0.0 &   \\
rc205 & OUR APPROACH & 569.4 & 630.2 & 630.2 & 34.1 & 69.3 &   \\
rc205 & BASELINE MILP & 366.8 & 630.2 & 630.2 & 95.5 & 0.0 &   \\
rc206 & OUR APPROACH & 521.2 & 610.0 & 610.0 & 153.6 & 133.2 & **** \\
rc206 & BASELINE MILP & 292.2 & 586.0 & 610.0 & 1000.0 & 0.0 & **** \\
rc207 & OUR APPROACH & 462.5 & 483.5 & 561.5 & 1000.0 & 692.5 &   \\
rc207 & BASELINE MILP & 255.3 & 341.7 & 560.2 & 1000.0 & 0.0 &   \\
rc208 & OUR APPROACH & 283.8 & 292.5 & 493.8 & 1000.2 & 1682.9 &   \\
rc208 & BASELINE MILP & 229.2 & 265.5 & 517.7 & 1000.0 & 0.0 &   \\
\bottomrule
\end{tabular}
\end{table}

==> old_tables.tex <==








\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
        \textbf{File ID} & \textbf{Approach} & \textbf{LP Obj} & \textbf{MILP LB} & \textbf{MILP Obj} & \textbf{MILP Time} & \textbf{LP Time} & \textbf{ 10X$<$} \\ \hline
        \textbf{r101} & LA-Discretization & 1047 & 1047 & 1047 & 0 & 0 & ~ \\ 
         & Baseline MILP & 1032 & 1047 & 1047 & 0 & 0 & ~ \\ \hline
        \textbf{r102} & LA-Discretization & 911 & 911 & 911 & 0 & 1 & YES \\ 
        & Baseline MILP & 652 & 911 & 911 & 51 & 0 & ~ \\ \hline
        \textbf{r103} & LA-Discretization & 765 & 776 & 776 & 2 & 11 & YES \\ 
         & Baseline MILP & 536 & 726 & 776 & 1000 & 0 & ~ \\ \hline
        \textbf{r104} & LA-Discretization & 615 & 631 & 631 & 53 & 75 & YES \\ 
         & Baseline MILP & 467 & 545 & 653 & 1000 & 0 & ~ \\ \hline
        \textbf{r105} & LA-Discretization & 901 & 914 & 914 & 0 & 1 & ~ \\ 
         & Baseline MILP & 795 & 914 & 914 & 1 & 0 & ~ \\ \hline
        \textbf{r106} & LA-Discretization & 795 & 795 & 795 & 0 & 4 & YES \\ 
         & Baseline MILP & 549 & 795 & 795 & 629 & 0 & ~ \\ \hline
        \textbf{r107} & LA-Discretization & 703 & 714 & 714 & 2 & 30 & YES \\ 
        & Baseline MILP & 486 & 634 & 714 & 1000 & 0 & ~ \\ \hline
        \textbf{r108} & LA-Discretization & 587 & 606 & 620 & 1000 & 106 & ~ \\ 
         & Baseline MILP & 460 & 533 & 634 & 1000 & 0 & ~ \\ \hline
        \textbf{r109} & LA-Discretization & 755 & 791 & 791 & 14 & 38 & YES \\ 
         & Baseline MILP & 550 & 771 & 791 & 1000 & 0 & ~ \\ \hline
        \textbf{r110} & LA-Discretization & 683 & 699 & 699 & 13 & 36 & YES \\ 
        & Baseline MILP & 483 & 613 & 699 & 1000 & 0 & ~ \\ \hline
        \textbf{r111} & LA-Discretization & 677 & 710 & 710 & 22 & 38 & YES \\ 
         & Baseline MILP & 478 & 608 & 711 & 1000 & 0 & ~ \\ \hline
        \textbf{r112} & LA-Discretization & 597 & 618 & 633 & 1000 & 166 & ~ \\ 
        & Baseline MILP & 455 & 520 & 655 & 1000 & 0 & ~ \\ \hline
    \end{tabular}
    \caption{\label{demo-table}50 Customers: Data set R101-112}
    \label{table_data_50}
\end{table}


\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
        \textbf{File ID} & \textbf{Approach} & \textbf{LP Obj} & \textbf{MILP LB} & \textbf{MILP Obj} & \textbf{MILP Time} & \textbf{LP Time} & \textbf{ 10X$<$} \\ \hline
        \textbf{c101} & LA-Discretization & 829 & 829 & 829 & 0 & 3 & ~ \\ 
         & Baseline MILP & 821 & 829 & 829 & 0 & 0 & ~ \\ \hline
        \textbf{c102} & LA-Discretization & 829 & 829 & 829 & 2 & 59 & ~ \\ 
        & Baseline MILP & 756 & 829 & 829 & 32 & 0 & ~ \\ \hline
        \textbf{c103} & LA-Discretization & 828 & 828 & 828 & 18 & 88 & YES \\ 
         & Baseline MILP & 590 & 812 & 829 & 1000 & 0 &  \\ \hline
        \textbf{c104} & LA-Discretization & 820 & 825 & 825 & 197 & 203 & YES \\ 
         & Baseline MILP & 578 & 675 & 826 & 1000 & 0 &  \\ \hline
        \textbf{c105} & LA-Discretization & 829 & 829 & 829 & 0 & 4 & ~ \\ 
         & Baseline MILP & 820 & 829 & 829 & 0 & 0 & ~ \\ \hline
        \textbf{c106} & LA-Discretization & 829 & 829 & 829 & 1 & 6 & ~ \\ 
        & Baseline MILP & 702 & 829 & 829 & 1 & 0 & ~ \\ \hline
        \textbf{c107} & LA-Discretization & 829 & 829 & 829 & 0 & 8 & ~ \\
         & Baseline MILP & 820 & 829 & 829 & 0 & 0 & ~ \\ \hline
        \textbf{c108} & LA-Discretization & 829 & 829 & 829 & 4 & 63 & ~ \\ 
         & Baseline MILP & 571 & 829 & 829 & 5 & 0 & ~ \\ \hline
        \textbf{c109} & LA-Discretization & 827 & 829 & 829 & 37 & 133 & YES \\ 
         & Baseline MILP & 567 & 795 & 829 & 1000 & 0  & ~ \\ \hline
    \end{tabular}
    \caption{100 Customers:  Data set C101-109}
    \label{table_data_100}

\end{table}

Updated tables:\\
